Characterizing quantum instruments: from non-demolition measurements to quantum error correction

In quantum information processing quantum operations are often processed alongside measurements which result in classical data. Due to the information gain of classical measurement outputs non-unitary dynamical processes can take place on the system, for which common quantum channel descriptions fail to describe the time evolution. Quantum measurements are correctly treated by means of so-called quantum instruments capturing both classical outputs and post-measurement quantum states. Here we present a general recipe to characterize quantum instruments alongside its experimental implementation and analysis. Thereby, the full dynamics of a quantum instrument can be captured, exhibiting details of the quantum dynamics that would be overlooked with common tomography techniques. For illustration, we apply our characterization technique to a quantum instrument used for the detection of qubit loss and leakage, which was recently implemented as a building block in a quantum error correction (QEC) experiment (Nature 585, 207-210 (2020)). Our analysis reveals unexpected and in-depth information about the failure modes of the implementation of the quantum instrument. We then numerically study the implications of these experimental failure modes on QEC performance, when the instrument is employed as a building block in QEC protocols on a logical qubit. Our results highlight the importance of careful characterization and modelling of failure modes in quantum instruments, as compared to simplistic hardware-agnostic phenomenological noise models, which fail to predict the undesired behavior of faulty quantum instruments. The presented methods and results are directly applicable to generic quantum instruments.

==> Quantum_instrument (Arxiv)/SupplementaryMaterial.tex <==
\onecolumngrid
\setcounter{figure}{0}
\setcounter{equation}{0}
\setcounter{table}{0}
\setcounter{section}{0}
\makeatletter 
\renewcommand{\theequation}{S\@arabic\c@equation}
\renewcommand{\thefigure}{S\@arabic\c@figure}
\renewcommand{\thetable}{S\@arabic\c@table}
\renewcommand{\RS}[1]{{\color{BLUE}{[RS]: #1}}}
\makeatother


\begin{center}
{\bf \large Supplementary Material: \\
Characterizing quantum instruments: \\
from non-demolition measurements to quantum error correction}
\label{SI}
\end{center}
\medskip
The additional information presented here aims at providing further experimental and theoretical results supporting our findings into more detail. We start by giving a broader insight on the experimental setup in Sec.~\ref{SISec:Toolbox}. Upon those building blocks we will be able to derive the maps underlying our quantum non-demolition (QND) loss detection unit for both asymmetric loss and the quantum erasure-channel. This will be complemented by further experimental data, both presented in section Sec.~\ref{SISec:QND}. We continue in Sec.~\ref{SISec:NoiseModel} by developing a noise model giving a well-founded description to our experimental limitations. Thereafter, those noise models form the basic building blocks to numerical simulations studying the implications of the loss detection in respect of quantum error correcting (QEC) codes. We conclude with Sec.~\ref{SISec:ColorCode} by giving more detailed derivations covering the loss treatment in the 7-qubit color code.

\section{Experimental details and toolbox}
\label{SISec:Toolbox}
Our ion-trap based quantum computer works on a chain of $^{40}$Ca$^+$ ions stably confined within ultra high vacuum using a linear Paul trap~\cite{toolbox}. Each ion represents a physical qubit encoded in the electronic levels $S_{1/2}(m=-1/2) = \ket{0}$ and $D_{5/2}(m=-1/2) = \ket{1}$ denoting the computational subspace. Qubit manipulation is realized by coherent laser-ion interaction. Thereby the setup is capable of implementing a universal set of quantum gate operations consisting of addressed single-qubit rotations with an angle $\theta$ around the x- and the y-axis of the form $\text{R}^\sigma(\theta) = \exp(-i{\theta}\sum_j {\sigma_j}/{2})$ with $\sigma = X$ or $Y$ together with two-qubit M\o{}lmer-S\o{}renson entangling gate operations $\text{MS}_{i,j}(\theta) = \exp(-i{\theta}\sum_{i,j} X_i X_j /2)$~\cite{MSgate}. Multiple addressed laser beams, coherent among themselves, allow for arbitrary two-qubit connectivity across the entire ion string. Read-out is performed by driving a dipole transition only resonant to the lower qubit level $\ket{0}$ and simultaneously collecting its scattered photons revealing the qubit's state after multiple shots. This dipole laser collectively covers the entire ion string. However, we are able to read out only a subset of the qubits within the register, by shelving electronic populations of specific qubits in the upper D-state manifold, referred to as addressed read out. Apart from quantum non-demolition measurements this becomes essential for reading out quantum trits (qutrits) demanding for two subsequent detections separating both levels $D_{5/2}(m=-1/2) = \ket{1}$ and $D_{5/2}(m=+1/2) = \ket{2}$, see~\cite{Ringbauer2021}. 

\section{Quantum Instrument: QND loss detection}
\label{SISec:QND}
This section gives a more thorough introduction to the QND-detection, serving as our quantum instrument working example, by deriving all maps relevant to our studies. Then, additional experiments are presented addressing the demonstration of the QND-detection's principal working ability complemented by results on the higher dimensional process tomography fully characterizing its underlying maps.

As loss on our setup naturally occurs on rates similar to those of single-qubit errors we introduce it in controlled fashion. For instance from the system qutrit's (q) state $\ket{0}_q$ loss can be induced by coherently transferring part of the population outside the computational subspace into $D_{5/2}(m=+1/2)=\ket{2}_q$ via the rotation
\begin{align}
\begin{split}
\mathrm{R}_\text{loss}(\phi) &= \ket{1}\bra{1}_q + \cos(\phi/2) (\ket{0}\bra{0}_q+\ket{2}\bra{2}_q) +\sin(\phi/2)(\ket{0}\bra{2}_q - \ket{2}\bra{0}_q).
\end{split}
\end{align}
The loss rate $\phi$ relates to the loss probability via $p_\text{loss}=\sin^2(\phi/2)$. Note that loss in general can be induced through an arbitrary state $\alpha\ket{0}_q+\beta\ket{1}_q$ with $\abs{\alpha}^2+\abs{\beta}^2=1$ using a single coherent rotation on the system qutrit before and its inverse after the loss rotation $R_\text{loss}(\phi)$. To detect loss two full entangling  $\text{MS}^X(\phi/2)\cdot\text{MS}^X(\phi/2)=\text{MS}^X(\phi)$ couple to ancilla and system qutrit and realize a collective bit-flip only if both qubits are present to their computational subspace:
 \begin{equation}
 \begin{split}
\text{MS}^X(\phi) &= \exp\big( - i\frac{\phi}{2} X_a X_q\big) =\Big(\cos(\phi/2)(\mathds{1}_a \otimes \mathds{1}_q - \ket{2}\bra{2}_q) 
-i \sin(\phi/2) X_a X_q\Big)+\ket{2}\bra{2}_q
\end{split}
\end{equation}
with 
\begin{align}
\begin{split}
\mathds{1}_a &=
\begin{pmatrix}
1&0\\
0&1\\
\end{pmatrix},
\hspace{0.3cm} \mathds{1}_q =
\begin{pmatrix}
1&0&0\\
0&1&0\\
0&0&1\\
\end{pmatrix},
\hspace{0.3cm}X_{a} =
\begin{pmatrix}
0&1\\
1&0\\
\end{pmatrix},\hspace{0.3cm} X_{q} =
\begin{pmatrix}
0&1&0\\
1&0&0\\
0&0&0\\
\end{pmatrix}.
\end{split}    
\end{align}
On the other hand if the system qutrit occupies a state outside the computational subspace, for instance in $\ket{2}_q$, the MS-gate is subject to an identity operation, which can be seen from the argument of its exponential $X_i X_i = \mathds{I}$ acting merely on the ancilla qubit. This follows a collective bit-flip
\begin{align}
\begin{split}
\mathrm{R}^X_a(\pi) &= -i (\ket{0}\bra{1}_a + \ket{1}\bra{0}_a ) \\ 
\mathrm{R}^X_q(\pi) &=\ket{2}\bra{2}_q -i (\ket{0}\bra{1}_q + \ket{1}\bra{0}_q )
\end{split}
\end{align}
Consequently, in the absence of loss the effect of the MS-gate is undone whereas under loss the ancilla qubit gets excited by the final bit-flip signaling the event of loss. The overall unitary combining loss operation and QND detection is given by
\begin{align}
\begin{split}
    U &= \mathrm{R}^X_a(\pi) \mathrm{R}^X_q(\pi)\mathrm{MS}^X(\pi)\mathrm{R_\text{loss}}(\phi)\\
    &=\mathds{1}_a \otimes U^{(0)}   + X_a \otimes U^{(1)}
\label{Eqn:SingleQutritQND}
\end{split}
\end{align}
with 
\begin{align}
\begin{split}
    U_q^{(0)} & =\ket{1}\bra{1}_q + \cos(\phi/2) \ket{0}\bra{0}_q + \sin(\phi/2) \ket{0}\bra{2}_q,   \\
    U_q^{(1)} & = \sin(\phi/2)\ket{2}\bra{0}_q - \cos(\phi/2) \ket{2}\bra{2}_q.
\end{split}
\end{align}
Taking the additional loss state $\ket{2}_q$ on the system qubit into account and by that extending the view from qubit to qutrit one ends up with two unitary processes fully describing this quantum instrument. We emphasize that on the qutrit level the entire dynamics of our detection unit can be captured, which is well exploited by the experiments from Fig.~\ref{Fig:QutritChois} in the main text of the paper.

However, to pick up the discussion on the non-unitary effects potentially leading to unwanted and erroneous mechanisms, we restrict our view again to the qubit level and further assume that no population was initially present in $\ket{2}_q$. Hence, the unitary operators $U_q^{(0)}$ and  $U_q^{(1)}$ reduce to the non-unitary ones
\begin{align}
\begin{split}
    A_q^{(0)} & =\ket{1}\bra{1}_q + \cos(\phi/2) \ket{0}\bra{0}_q, \\
    A_q^{(1)} & = \sin(\phi/2)\ket{2}\bra{0}_q.
\end{split}
\end{align}
leading to single qubit processes describing the QND detection restricted to the system qubit. We can describe both maps $\lbrace A_q^{(0)},A_q^{(1)}\rbrace$ by two trace non-increasing completely-positive (CP) maps $\mathcal{E}_0$ and $\mathcal{E}_1$.
\begin{align}
\begin{split}
    \mathcal{E}_0\colon \rho \mapsto A_q^{(0)}\rho A_q^{(0)\dag} \\
    \mathcal{E}_1\colon \rho \mapsto A_q^{(1)}\rho_q A_q^{(1)\dag} 
\end{split}
\end{align}
acting on the system qubits as 
\begin{equation}
    \rho \mapsto \ket{0}\bra{0}_a \otimes \mathcal{E}_0(\rho)   +   \ket{1}\bra{1}_a \otimes \mathcal{E}_1(\rho)
\label{Eqn:SingleQND}
\end{equation}
where the two maps are together unitary again. It is noteworthy that the no-loss map $\mathcal{E}_0$ initially starting from the superposition state $1/\sqrt{2}(\ket{0}_q+\ket{1}_q)$ would be transitioning to $\ket{1}_q$ as the loss probability from $\ket{0}_q$ increases, which is subject to Fig.~\ref{Fig:SingleQND_Bloch}a in the main text. Only for very little loss $\phi\sim 0$ the no-loss map converges to an identity operation. 

Next to having loss asymmetrically with respect to either computational basis state $\lbrace\ket{0}_q,\Ket{1}_q\rbrace$, we follow a different, often utilized, scenario called the quantum erasure-channel~\cite{Grassl1997}. Its circuit is depicted in Fig.~\ref{Fig:QInstrument}c from the main text. First, partial loss is induced from $\ket{0}_q$ followed by its detection. The protocol only continues in the absence of loss by inducing the same partial loss from the other qubit state $\ket{1}_q$ together with its detection. The second part of the map can be expressed via $\lbrace\tilde{A}_q^{(0)},\tilde{A}_q^{(1)}\rbrace$ where we swap the role of $\ket{0}_q$ and $\ket{1}_q$. Thus, the quantum erasure-channel can be described using the following map
\begin{align}
\begin{split}
    \rho \mapsto  & (1-p_L)  (1-\widetilde{p}_L)\widetilde{A}_q^{(0)} A_q^{(0)}  \rho A_q^{(0)\dag} \widetilde{A}_q^{(0)\dag}\\
    &+ (1-p_L) \widetilde{p}_L \widetilde{A}_q^{(1)}  \rho \widetilde{A}_q^{(1)\dag}  + p_L A_q^{(1)}  \rho A_q^{(1)\dag}
\end{split}
\end{align}
with probabilities $p_L$ and $\widetilde{p}_L$ for any arbitrary input state $\alpha\ket{0}_q + \beta\ket{1}_q $
\begin{equation}
p_L = \abs{\alpha}^2 \sin^2(\phi/2) \qquad
\widetilde{p}_L = \frac{\abs{\beta}^2 \sin^2(\phi/2)}{(\abs{\alpha}^2\cos^2(\phi/2) + \abs{\beta}^2)}.
\end{equation}
In this case the process reduces to
\begin{equation}
    \rho \mapsto  \cos^2(\phi/2) \rho + \sin^2(\phi/2) \ket{2}\bra{2}_q,
\label{Eqn:Erasure}
\end{equation}  
where the effect of the loss is proportional to the arbitrary input state $\rho$ indicating that after normalization the initial state can be retrieved independent of the loss probability.

The basic idea of this quantum instrument is the detection of qubit loss, i.e unwanted leakage to levels outside the computational subspace, that in a realistic scenario would be followed by its correction representing the scope of our foregoing work~\cite{Stricker2020}. To give the rather formal discussion a physical meaning, we demonstrate the unit's working principle. Partial loss induced from $\ket{0}_q$ via the loss transition $R_\text{loss}(\phi)$ is continuously increased and subsequently detected. Note that both qubits are read out denoting their population in the upper $\ket{D}$-state manifold referring to directly measured loss in case of the system qubit and detected loss for the ancilla qubit. In Fig.~\ref{SIFig:QNDTest} results are presented for individual and repeated loss detection employing up to two ancilla qubits. Slopes extracted from the linear-fit in the repeated detection read $0.938(9)$ and $0.944(12)$ for ancilla $a_1$ and $a_2$ respectively. On the individual read-outs we get $0.977(2)$ and $0.995(2)$ with a resonant cross-talk to the ancilla not participating of $0.005(1)$ and $0.003(1)$ respectively. When utilizing $a_2$ we end up with a higher detection efficiency because of a better performing MS-gate on the particular ion-pair. 200 cycles were taken on this measurement. Errors correspond to one standard deviation of statistical uncertainty due to quantum projection noise.

\begin{figure}[ht]
\centering
\includegraphics[width=\textwidth]{Figures/S1_QNDRabiFlops.pdf}
\caption{\textbf{Investigating the performance of the QND-detection unit according to Fig.~\ref{Fig:QInstrument}b in the main text.} Population in the D$_{5/2}$ state for the system qubit (directly measured loss) vs. transferred excitation on the ancilla qubit (detected loss) in case of detecting loss repeatedly using both ancilla qubits $a_1$ and $a_2$ (left), solely with ancilla $a_1$ (middle) and ancilla $a_2$ (right). The imprinted detection efficiencies demonstrate reliable loss mapping onto the ancilla qubit and its read out by means of QND. Errors correspond to one standard deviation of statistical uncertainty due to quantum projection noise.}
\label{SIFig:QNDTest}
\end{figure}

Next, we complement the results from  Fig.~\ref{Fig:SingleQND_Bloch}a in the main part revealing a pull towards the state not affected from asymmetric loss by further demonstrating that the purity $\Tr(\rho^2)$ of the associated reconstructed states remains constant across the entire loss probability range; see Fig.~\ref{SIFig:QNDPurity}a. The purity value is found independent of the loss and therefore underlining at first glance a correct experimental outcome whereas only in the Bloch sphere picture (Fig.~\ref{Fig:SingleQND_Bloch}a) deviations due to the non-unitary map become visible. Likewise considerations have been done on the erasure-channel, previously discussed in Fig.~~\ref{Fig:SingleQND_Bloch}b and similarly producing purity values independent of loss, as can be seen in Fig~\ref{SIFig:QNDPurity}b. 

\begin{figure}[ht]
\includegraphics[width=0.8\textwidth]{Figures/S2_QNDPurity.pdf}
\caption{\textbf{Purity of a single system qubit after undergoing the QND-detection in the no-loss case for different loss channels}. \textbf{(a)} After a single QND-detection with loss from $\ket{0}_q$ we find purity values unaffected by the amount of loss for all of the given input states. At high loss probabilities, tomography becomes unreliable due to the low count rates. \textbf{(b)} The erasure-channel is realized by consecutively inducing the same partial from $\ket{0}_q$ followed by $\ket{1}_q$ and post-selecting to both ancilla $\ket{0}_a$ outcomes. The purity of the output state is again unaffected by loss for any of the probed input states. Errors correspond to one standard deviation of statistical uncertainty due to quantum projection noise.}
\label{SIFig:QNDPurity}
\end{figure}

Next, we estimate the detection correlation of a single loss event by two repeated detections. Such system capabilities emphasize the work on the erasure-channel and more generally become relevant in a realistic scenario demanding several consecutive read-outs especially when embedded in QEC codes. In Fig.~\ref{SIFig:QNDRepeatability} positive correlation occurs for a certain shot when both ancilla qubits agree upon a certain loss event. Further, the data on the repeated read-out allows us to quantify false-positive and false-negative rates manifesting important failure modes of our detection unit. Again, false-positive rates dominate owing to their strong sensitivity on the entangling MS-gate as was the case in Fig.~\ref{Fig:QutritChois}b in the main text. 100 cycles for $\ket{0}_q$-loss and 200 cycles for $1/\sqrt{2}(\ket{0}_q+\Ket{1}_q)$-loss were taken on this measurement. Errors correspond to one standard deviation of statistical uncertainty due to quantum projection noise.

\begin{figure}[ht]
\centering
\includegraphics[width=1.0\textwidth]{Figures/S3_QNDCorrelations.pdf}
\caption{\textbf{Correlations between two repeated QND detections according to Fig.~\ref{Fig:QInstrument}b in the main text.} Loss on the system qubit was induced from the imprinted states followed by two repeated detections using ancilla $a_1$ and $a_2$. A Positive correlation refers to successfully detecting the same loss event twice, whereas faulty assignments can be separated in false-positive and false-negative events; shown in the lower figure part. Errors correspond to one standard deviation of statistical uncertainty due to quantum projection noise.}
\label{SIFig:QNDRepeatability}
\end{figure}

\begin{figure}[ht]
\includegraphics[width=\textwidth]{Figures/S4_ProcTomSchematics.pdf}
\caption{\textbf{Schematics on higher dimensional process tomography}. \textbf{(a)} Qutrit process tomography solely covering the system qubit $(q)$ together with the loss level $\lbrace\ket{0}_q,\ket{1}_q,\ket{2}_q\rbrace$ undergoing the QND-detection unit by using 9 preparation settings together with 6 measurement settings resulting in 54 experiments each run. \textbf{(b)} Combined process tomography on ancilla $(a)$ and qutrit $(1)$ capturing the entire dynamics of this quantum instrument using 12 settings on the ancilla qubit (4 preparation settings and 3 measurement settings) alongside 54 settings on the system qutrit resulting in 648 experiments. \textbf{(c)} Qutrit process tomography on the erasure-channel focusing on the no-loss case, i.e. twice post-selecting the ancilla qubit's $\ket{0}_a$ outcome.}\label{SIFig:Tomography_Schematics}
\end{figure}

We switch our consideration from qubit to qutrit level and resume the discussion on the process tomography covering both ancilla qubit and system qurtrit from Fig.~\ref{Fig:QutritChois}a in the main text. Thereby, all presented Choi-operators were post-selected upon the ancilla outcome denoting the qutrit maps separated by both loss-cases. This has the advantage of unitary operators describing the full dynamics of the system qutrit in either loss case that moreover gave an estimation on the QND detection's dominant failure mode, namely false-positive and false-negative rates. 
As discussed in detail in the main part of the paper standard tomography restricted to qubit level prevents us from getting such fine-grained analysis for mainly two reasons: First, reliably assigning false-positive and false-negative events is not possible when post-selecting by the ancilla qubit's measurement outcome. Second, when tracing over the ancilla the loss state $\ket{2}_q$ is incoherently added to the qubit state $\ket{1}_q$ creating an unphysical bias under which tomography is likely to break as demonstrated in Fig.~\ref{SIFig:QubitChoiTraced}. Here, we distinguish between tracing before and after tomography reconstruction. On the one hand, when directly tracing on the raw data and subsequently reconstructing the map it includes coherences owing to the reconstruction technique forcing physical properties. On the other hand, when tracing after process reconstruction coherences on $\ket{01}_q$ vanish. Both cases draw attention to potential risks on how commonly known process tomography fails to describe quantum instruments.

\begin{figure}[ht]
\centering
\includegraphics[width=0.8\textwidth]{Figures/S5_QutritTraced.pdf}
\caption{\textbf{Potential risks on system qubit process reconstruction when partial tracing the ancilla qubit}. \textbf{(left column)} Partial tracing before reconstructing the map directly on the raw data, previously used in Fig.~\ref{Fig:QutritChois} of the main part. In this case, the loss level $\ket{2}_q$ is incoherently added onto state $\ket{1}_q$. Coherences present in $\ket{01}_q$ originate from the reconstruction technique forcing physical properties. \textbf{(right column)} Post-selecting from the already reconstructed qubit-qutrit maps presented in Fig.~\ref{SIFig:QubitQutrit}. In contrast to before coherences on $\ket{01}_q$ vanish, whereas the unphysical bias remains.}
\label{SIFig:QubitChoiTraced}
\end{figure}

In the context of the numerical simulations covering implications on QEC however, we made use of the full map capturing the combined ancilla-qutrit dynamics together with the noise-models; further discussed below. We present experimentally estimated ancilla-qutrit Choi-operators for various loss probabilities in Fig.~\ref{SIFig:QubitQutrit} using the elementary basis according to $\lbrace\ket{0000}_{a,q},...,\ket{1212}_{a,q}\rbrace$. The process tomography of every loss probability required $54\times12=648$ experimental settings. For the sake of clarity we plot ideal Choi-operators (left column) and the experimental ones (right column) for various loss probabilities separated by rows side by side. Color and saturation refer to argument and absolute value of the complex matrix entries. Process fidelities with the ideal Choi-operator from top to bottom read $\lbrace 0.91(1), 0.89(1), 0.85(1)\rbrace$ referring to the loss probabilities $\lbrace \SI{0}{\%}, \SI{50}{\%}, \SI{85}{\%}\rbrace$. 100 cycles were taken for each experiment. In the no-loss case the expected controlled $\hat{X}_a$ operation signaling a loss event whenever the system qubit occupies level $\ket{2}_q$ is clearly reproduced as expressed by Eq.~\eqref{Eqn:SingleQutritQND} derived in the beginning of this section.

\begin{figure}[ht]
\centering
\includegraphics[width=\textwidth]{Figures/S6_QubitQutritChoi.pdf}
\caption{\textbf{Combined process reconstruction on ancilla-qutrit according to Fig.~\ref{SIFig:Tomography_Schematics}b}. The resulting Choi-operators (right column) denoted in elementary basis ($\lbrace\ket{0000}_{a,q},...,\ket{1212}_{a,q}\rbrace$) describe the whole dynamics of the QND-detection unit under loss from $\ket{0}_q$. Hue relates to phase according to the top right color bar and saturation to the absolute value of the complex entries. Process fidelities with the ideal Choi-operators (left column) from top to bottom read $\lbrace 0.91(1), 0.89(1), 0.85(1)\rbrace$. Errors correspond to 1 standard deviation of statistical uncertainty due to quantum projection noise.}
\label{SIFig:QubitQutrit}
\end{figure}

Finally, we present additional data on the system qutrit process tomography according to Fig.~\ref{SIFig:Tomography_Schematics}a and loss induced from $\ket{0}_q$ and $\ket{1}_q$ presented in Fig.~\ref{SIFig:SingleQNDQutrit} and Fig.~\ref{SIFig:SingleQNDQutritD} respectively. We emphasize that here similar to the qubit level certain coherences vanish when tracing over the ancilla, which is no longer covered by the process tomography. Still, the dynamics on the system qutrit clearly captures the population transfer from either basis state $\lbrace\ket{0}_q,\ket{1}_q\rbrace$ to the loss level $\ket{2}_q$. Further, a change in the asymmetric behaviour between loss from $\ket{0}_q$ and $\Ket{1}_q$ becomes distinctly visible in the qubit subspace.

\begin{figure}[ht]
\centering
\includegraphics[width=0.8\textwidth]{Figures/S7_QNDSloss.pdf}
\caption{\textbf{Qutrit process tomography characterizing the QND-detection unit for loss from $\ket{0}_q$ according to Fig.~\ref{SIFig:Tomography_Schematics}a}. \textbf{(a)} System qutrit's Choi-operator in elementary basis $\lbrace\ket{00}_q,...,\ket{22}_q\rbrace$ after tracing over the ancilla qubit and various loss probabilities denoting the effect of the loss-transition transferring population from $\ket{0}_q$ to $\ket{2}_q$. \textbf{(b)} The respective fidelities with the ideal Choi-operators covering the complete loss range.}
\label{SIFig:SingleQNDQutrit}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.8\textwidth]{Figures/S8_QNDDloss.pdf}
\caption{\textbf{Qutrit process tomography characterizing the QND-detection unit for loss from $\ket{1}_q$ according to Fig.~\ref{SIFig:Tomography_Schematics}a}. \textbf{(a)} System qutrit's Choi-operator in elementary basis $\lbrace\ket{00}_q,...,\ket{22}_q\rbrace$ after tracing over the ancilla qubit and several different loss probabilities denoting the effect of the loss-transition transferring population from $\ket{1}_q$ to $\ket{2}_q$. \textbf{(b)} The respective fidelities compared to the ideal Choi-operators covering the complete loss range.}
\label{SIFig:SingleQNDQutritD}
\end{figure}

For the sake of completeness we present similar Choi-operators on the repeated loss detection in Fig.~\ref{SIFig:RepeatedQNDQutrit} consecutively mapping the same loss event to two different ancilla qubits; shown for loss from $\ket{0}_q$. As the reconstructed Choi-operators follow the expected behaviour previously observed, their fidelities turn out slightly lower compared to Fig.~\ref{SIFig:SingleQNDQutrit} as expected due to the more complex experiment. 

\begin{figure}[ht]
\centering
\includegraphics[width=0.8\textwidth]{Figures/S9_2QNDsSloss.pdf}
\caption{\textbf{Qutrit process tomography on two repeated QND-detections for loss from $\ket{0}_q$ according to Fig.~\ref{SIFig:Tomography_Schematics}a}. \textbf{(a)} System qutrit Choi-operators mapping loss repeatedly onto ancilla $a_1$ and $a_2$ under several different loss probabilities. The processes for which we traced over both ancillas prior to reconstruction denote the loss-transition transferring population from $\ket{0}_q$ to $\ket{2}_q$. \textbf{(b)} Fidelities compared to the ideal operators remain approximately constant along all measured loss probabilities and show slightly decrased values compared to the results on the single QND detection from Fig.~\ref{SIFig:SingleQNDQutrit}.}
\label{SIFig:RepeatedQNDQutrit}
\end{figure}


\section{Noise model on QND loss detection}
\label{SISec:NoiseModel}

\begin{figure}[ht]
\centering
\includegraphics[width=0.85\textwidth]{Figures/S10_NoiseModels.pdf}
\caption{\textbf{Noise-models QND-detection}. Various noise-models describing the experimental limitations on the ancilla-qutrit Choi-operator depicted in Fig.~\ref{SIFig:QubitQutrit}. The limitations are best described when combining correlated coherent rotations together with depolarizing and dephasing noise. Correlated errors clearly dominate as depolarizing and dephasing errors only lead to minor improvements. The error parameters on the bottom of each plot refer to depolarizing error $p_\text{depol.}$, dephasing error $p_\text{deph.}$ and correlated error $p_\text{corr.}$, the latter according to Eq.~\eqref{SIEq:CorrelatedNoiseModel}. Lines are connecting the points for clarity.}
\label{SIFig:NoiseModel}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.95\textwidth]{Figures/S11_NoiseModelsChois}
\caption{\textbf{Comparison between experimental and noisy modeled Choi-operators}. \textbf{(a)} Experimentally estimated map according to Fig.~\ref{SIFig:QubitQutrit}a with additionally marked transitions denoting correlated errors describing our leading error mechanism, see Eq.~\eqref{SIEq:CorrelatedNoiseModel}. \textbf{(b)} Most suitable noisy modelled Choi-operator combining correlated, depolarizing and dephasing errors.}
\label{SIFig:NoiseModelChoi}
\end{figure}

\begin{table}[ht]
\centering
\begin{tabular}{c c c c c c c c c c c c}
    \toprule
    \midrule
    \multirow{1}[4]{*}{} & \multirow{1}[4]{*}{} & \multicolumn{2}{c}{depolarizing} & \multicolumn{2}{c}{dephasing} & \multicolumn{2}{c}{correlated} & \multicolumn{4}{c}{correlated, depol. and dephas.} \\ 
    \cmidrule(rl){1-1}\cmidrule(rl){2-2}\cmidrule(rl){3-4}\cmidrule(rl){5-6}\cmidrule(rl){7-8}\cmidrule(rl){9-12}
   loss & $\mathcal{F}_\text{ideal}$ & $\mathcal{F}_\text{model}$ & $p_\text{depol.}$ &   $\mathcal{F}_\text{model}$ & $p_\text{deph.}$ & $\mathcal{F}_\text{model}$ & $p_\text{corr.}$ & $\mathcal{F}_\text{model}$ & $p_\text{corr.}$ & $p_\text{depol.}$ & $p_\text{deph.}$ \\ 
        \cmidrule(rl){1-1}\cmidrule(rl){2-2}\cmidrule(rl){3-4}\cmidrule(rl){5-6}\cmidrule(rl){7-8}\cmidrule(rl){9-12}
    \multicolumn{1}{r}{\SI{0}{\%}}  & 0.906 & 0.912 & 0.004 & 0.915 & 0.013 & 0.939 & 0.045 & 0.948 &  0.042 & 0.012 & 0.002\\
    \multicolumn{1}{r}{\SI{2}{\%}}  & 0.899 & 0.912 & 0.009 & 0.908 & 0.014 & 0.916 & 0.021 & 0.923 & 0.045 & 0.010 & 0.010\\ 
    \multicolumn{1}{r}{\SI{50}{\%}}  & 0.894 & 0.905 & 0.007 & 0.905 & 0.018 & 0.924 & 0.032 & 0.934 & 0.037 & 0.020 & 0.007\\
    \multicolumn{1}{r}{\SI{85}{\%}}  & 0.854 & 0.861 & 0.005 & 0.863 & 0.017 & 0.897 & 0.054 & 0.903 & 0.045 & 0.010 & 0.010\\
    \midrule
    \bottomrule
\end{tabular}
\caption{\textbf{Summary on noise model parameters and results}: The parameters and fidelities refer to the best suitable model values describing the experimental noise from Fig.~\ref{SIFig:NoiseModel}: depolarizing error $p_\text{depol.}$, dephasing error $p_\text{deph.}$ and correlated error $p_\text{corr.}$ according to Eq.~\eqref{SIEq:CorrelatedNoiseModel}.}
\label{SITab:Params}
\end{table}

Here, we study various noise models in order to find the best suitable description of the experimental limitations underlying our QND-detection. Although very small contributions will be precluded by state preparation and measurement errors (SPAM-errors) the resulting models give us a rough estimate as a guide for where to look at upon which a microscopic noise model for the numerical simulations can be developed. Getting more insights on these error mechanisms is essential when observing implications of the quantum instrument in context of QEC protocols and is further an essential building block towards fault-tolerant quantum computation; see implication on QEC section in the main text. 

We refer to Eq.~\eqref{Eqn:SingleQutritQND} from above and express the action of the ideal QND map $U$ under a given loss rate $\phi$ acting on the combined ancilla-qutrit system in terms of the Choi operator $\rho^\text{CJ} = \mathds{1} \otimes U \cdot\ket{\Phi_+}\bra{\Phi_+}\cdot\mathds{1} \otimes  U^\dagger$ where $\ket{\Phi_+}\bra{\Phi_+}$ is the maximally entangled state of two copies of the ancilla-qutrit system.  An erroneous channel $\mathcal{E}_\text{noise}$ transforms the Choi operator $\rho^{\text{CJ}}$ to  $\rho^\text{CJ}_\text{noise} = (\mathds{1} \otimes \mathcal{E}_\text{noise})( \rho^\text{CJ} )$. Noise rates entering $\mathcal{E}_\text{noise}$ for given model parameters are then extracted by minimizing the distance between modelled noisy Choi-operators $\rho^\text{CJ}_\text{noise}$ and the experimentally determined ones $\rho^\text{CJ}_\text{exp}$ from Fig.~\ref{SIFig:QubitQutrit}. As a measure for the distance in the cost-function we minimize the infidelity:
\begin{equation}
\vert\vert 1-\mathcal{F}(\rho^\text{CJ}_\text{exp}, \rho^\text{CJ}_\text{noise})\vert\vert.
\end{equation}
Our initial considerations covered the study of the QND detection's failure modes, i.e.~false-positive and false-negative rates both quantified in the main part of the paper. Measuring process tomography however comes along with overhead in the form of preparation and measurement gates followed by two consecutive detections at the end of each experiment required for reading out the qutrit's state. Therefore SPAM errors are not to be neglected and lead to a significant bias on false-positive and false-negative rates. With this in mind we put the failure modes aside and focus on experimental limitations instead. In the following, we consider as model for $\mathcal{E}_\text{noise}$ a depolarizing, a dephasing channel, and coherent two- and single-qubit overrotations.

\textbf{Depolarizing and dephasing channels}.--- We start off by testing the agnostic models, namely depolarizing and dephasing channels as those represent error mechanisms typically considered in the field of quantum computation~\cite{NielsenChuang}. The effect of the latter can be understood by losing phase information between the quantum states involved. Coherences get lost and an arbitrary single qubit state in the Bloch sphere picture would finally shrink onto the $Z$-axis as no phase information is left. Depolarizing noise can be considered as simultaneous dephasing in $X$, $Y$ and $Z$ basis eventually leading to a complete mixed state which for a single qubit can be illustrated by shrinking the Bloch sphere towards its center. Note that, we implement those models such that they act both on the ancilla and the qutrit using only a single noise parameter~\cite{Wei2013}. The upper row of Fig.~\ref{SIFig:NoiseModel} depicts the fidelities (top part) for the individual models at the optimized parameters (bottom part). Both results indicate similar improvements compared to the fidelity with the ideal QND map from Eq.~\eqref{Eqn:SingleQutritQND}. Numbers on fidelities and optimized parameters for depolarizing noise $p_\text{depol.}$ and dephasing noise $p_\text{deph.}$ are further summarized in Tab.~\ref{SITab:Params}. The parameters typically lie around 1\% or below, yet the small increase in fidelity indicates other error mechanisms to be more dominant. 

\textbf{Correlated two-qubit overrotations}.---The erroneous peaks in the experimentally estimated Choi-operators from Fig.~\ref{SIFig:QubitQutrit} imply that additional rotations should be taken into account by the agnostic models. Those dominant error peaks are found originating from correlated rotations between ancilla and system qubit as illustratively labeled in Fig.~\ref{SIFig:NoiseModelChoi}a. Note that the error terms are restricted to qubit level and partial coherences are still present. Hence, if the system qutrit's state is~$\ket{2}_q$ no correlated error is induced on the ancilla qubit. Therefore, correlated errors are due to faulty entangling MS-gates. A potential noise model covering correlated rotations in such a way reads:
\begin{equation}
\rho \mapsto \mathcal{E}_\text{noise}(\rho) =  U_\text{corr} \rho U_\text{corr}^{\dag}
\end{equation}
with
\begin{align}
\begin{split}
 U_\text{corr} &= \cos\frac{\alpha}{2}\ \mathds{1}_a\otimes\mathds{1}_q +i \sin\frac{\alpha}{2} \ (X_a\otimes X_{q}+\mathds{1}_a\otimes\ket{2}\bra{2}_q) 
\label{SIEq:CorrelatedNoiseModel}
\end{split}
\end{align}
where $\alpha$ describes the correlated under-/ overrotations and relates to the corresponding error probability via $p_\text{corr.}=\sin(\alpha/2)^2$. For comparison a value  $p_\text{corr.}$ of $0.5$ would induce a maximally entangling two-qubit operation on ancilla and system qubit. We first test the model alone followed by combining it with depolarizing and dephasing noise. The resulting fidelities (top part) at the optimized model parameters (bottom part) are shown in the second row of Fig.~\ref{SIFig:NoiseModel} and clearly overcome the ones on the agnostic models denoting correlated rotations to be our leading noise mechanism. The effect of the additional depolarizing and dephasing noise (bottom right) leads to slight improvements. The modeled Choi-operator on this combined noise model is plotted for the no-loss case in Fig.~\ref{SIFig:NoiseModelChoi}b showing strong similarities to the experimental one from part a underlining a good agreement between model and experiment. Numbers on fidelities and optimized parameters for all models are summarized in Tab.~\ref{SITab:Params}.

\textbf{Correlated and single overrotations}.---Finally, we combine the action of correlated rotations with single-qubit rotations on the ancilla and the qutrit and we consider the coherent error model given by
\begin{equation}\label{SIEqn:CorrelatedSingleRotationChannel}
\rho \mapsto \mathcal{E}_\text{noise}(\rho) =  {R}\ U_\text{corr} \rho U_\text{corr}^{\dag} \ {R}^{\dag}
\end{equation}
where $\rho$ is the state obtained after the application of the loss operation $U$ of Eq.~\eqref{Eqn:SingleQutritQND} (see also Fig.~\ref{Fig:7QubitCode}a of the main text), $U_\text{corr}$ is a correlated two-qubit overrotation defined in Eq.~\eqref{SIEq:CorrelatedNoiseModel} and $R = \mathrm{R}^X_a(\beta) \mathrm{R}^X_q(\beta)$ with
\begin{gather}\label{eqn_rotation_x_a}
R^X_a(\beta) = \cos (\beta / 2) - i\sin (\beta / 2) X_a \\ 
R^X_q(\beta) = \cos (\beta / 2)(1 - \ket{2}\bra{2}_q)  - i\sin (\beta / 2) X_q + \ket{2}\bra{2}_q  \label{eqn_rotation_x_q} 
\end{gather}
are overrotations with angle $\beta$ of the ancilla and the qutrit system which corresponds to the single qubit flip error rate $p_\text{single} = \sin(\beta / 2)^2$. After the measurement of the ancilla, the quantum process arising from the erroneous channel in Eq.~\eqref{SIEqn:CorrelatedSingleRotationChannel} can be written as
\begin{equation}\label{eqn_supp_coherent_channel}
\rho \mapsto \ket{0}\bra{0}_a \otimes \mathcal{R}_0(\rho_q)  +  \ket{1}\bra{1}_a \otimes \mathcal{R}_1(\rho_q)
\end{equation}
where $\rho_q$ is the state related to the qutrit only and the processes $\mathcal{R}_0$ and $\mathcal{R}_1$ describe the maps that transform the qutrit state in the case of no-loss detected (ancilla qubit in $\ket{0}_a$) and of loss detected (ancilla qubit in $\ket{1}_a$).  The Choi operators $\Lambda_0$ and $\Lambda_1$ of the maps $\mathcal{R}_0$ and $\mathcal{R}_1$ can be computed for all values of the over-rotated angles $\alpha$ and $\beta$. In particular, if we consider small deviations for  $\alpha$ and $\beta$, $\Lambda_0$ and $\Lambda_1$ read at second order

\colorlet{gray_1}{green!10}
\colorlet{gray_2}{blue!10}
\colorlet{gray_3}{red!30}
\colorlet{gray_4}{magenta!30}
\colorlet{gray_5}{orange!30}
\colorlet{gray_6}{teal!30}

\newcommand{\grayone}[1]{%
  \begingroup\setlength{\fboxsep}{0pt}% no padding
  \colorbox{gray_1}{#1}%
  \endgroup
}
\newcommand{\graytwo}[1]{%
  \begingroup\setlength{\fboxsep}{0pt}% no padding
  \colorbox{gray_2}{#1}%
  \endgroup
}
\newcommand{\graythree}[1]{%
  \begingroup\setlength{\fboxsep}{0pt}% no padding
  \colorbox{gray_3}{#1}%
  \endgroup
}
\newcommand{\grayfour}[1]{%
  \begingroup\setlength{\fboxsep}{0pt}% no padding
  \colorbox{gray_4}{#1}%
  \endgroup
}

\newcommand{\grayfive}[1]{%
  \begingroup\setlength{\fboxsep}{0pt}% no padding
  \colorbox{gray_5}{#1}%
  \endgroup
}

\newcommand{\graysix}[1]{%
  \begingroup\setlength{\fboxsep}{0pt}% no padding
  \colorbox{gray_6}{#1}%
  \endgroup
}
{\small
\begin{equation}
\Lambda_0 = 
\left(
\begin{array}{ccccccccc}
\cellcolor{gray_1} 1 -\frac{\alpha ^2}{4} - \frac{\beta^2}{2}& \left(-\frac{\alpha }{4}-\frac{i}{2}\right) \beta  & 0 & \left( -\frac{\alpha }{4}-\frac{i}{2}\right) \beta  & 1 -\frac{\alpha ^2}{4} - \frac{\beta^2}{2}& 0 & 0 & 0 & \frac{i}{2}  \beta  \\
 \left(-\frac{\alpha }{4}+\frac{i}{2}\right) \beta  & \cellcolor{gray_2} \frac{\beta ^2}{4} & 0 & \frac{\beta ^2}{4} & \left(-\frac{\alpha }{4}+\frac{i}{2}\right) \beta  & 0 & 0 & 0 & -\frac{1}{4} \beta ^2 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 \left( -\frac{\alpha }{4}+\frac{i}{2}\right) \beta  & \frac{\beta ^2}{4} & 0 & \cellcolor{gray_2}\frac{\beta ^2}{4} & \left(-\frac{\alpha }{4}+\frac{i}{2}\right) \beta  & 0 & 0 & 0 & -\frac{1}{4}\beta^2 \\
1 -\frac{\alpha ^2}{4} - \frac{\beta^2}{2} & \left(-\frac{\alpha }{4}-\frac{i}{2}\right) \beta  & 0 & \left(-\frac{\alpha }{4}-\frac{i}{2}\right) \beta  & \cellcolor{gray_1} 1 -\frac{\alpha ^2}{4} - \frac{\beta^2}{2} & 0 & 0 & 0 & \frac{i}{2} \beta  \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
  -\frac{i}{2} \beta  & -\frac{1}{4} \beta ^2 & 0 & -\frac{1}{4} \beta ^2 &  -\frac{i}{2} \beta  & 0 & 0 & 0 & \cellcolor{gray_3} \frac{\beta ^2}{4} 
\end{array}
\right)
\end{equation}

\begin{equation}
\Lambda_1 = 
\left(
\begin{array}{ccccccccc}
\cellcolor{gray_5} \frac{\beta ^2}{4} & \frac{\alpha  \beta }{4} & 0 & \frac{\alpha  \beta }{4} & \frac{\beta ^2}{4} & 0 & 0 & 0 & \left(\frac{\alpha }{4}-\frac{i}{2}\right) \beta  \\
 \frac{\alpha  \beta }{4} & \cellcolor{gray_4}\frac{\alpha ^2}{4} & 0 & \frac{\alpha ^2}{4} & \frac{\alpha  \beta }{4} & 0 & 0 & 0 & \frac{\beta ^2}{4}-\frac{i \alpha }{2} \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 \frac{\alpha  \beta }{4} & \frac{\alpha ^2}{4} & 0 & \cellcolor{gray_4}\frac{\alpha ^2}{4} & \frac{\alpha  \beta }{4} & 0 & 0 & 0 & \frac{\beta ^2}{4}-\frac{i \alpha }{2} \\
 \frac{\beta ^2}{4} & \frac{\alpha  \beta }{4} & 0 & \frac{\alpha  \beta }{4} & \cellcolor{gray_5}\frac{\beta ^2}{4} & 0 & 0 & 0 & \left(\frac{\alpha }{4}-\frac{i}{2}\right) \beta  \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 \left(\frac{\alpha }{4}+\frac{i}{2}\right) \beta  & \frac{\beta ^2}{4}+\frac{i \alpha }{2} & 0 & \frac{\beta ^2}{4}+\frac{i \alpha }{2} & \left(\frac{\alpha }{4}+\frac{i}{2}\right) \beta  & 0 & 0 & 0 & \cellcolor{gray_6} 1-\frac{\beta ^2}{4} \\
\end{array}
\right)
\end{equation}
}
where we have labeled the qutrit basis states in the order $\ket{00}, \ket{01}, \ket{02}, \dots \ket{22}$. In the next section we discuss how to approximate the channel in Eq.~\eqref{eqn_supp_coherent_channel} with Clifford gates.


\textbf{Effective Clifford channel}.---Before deriving the analytical expression for the Clifford channel, the form of Choi operators $\Lambda_0$ and $\Lambda_1$ allows us to make a qualitative discussion on the events that will form the Clifford channel approximating Eq.~\eqref{eqn_supp_coherent_channel}. In $\Lambda_0$ and $\Lambda_1$ we can easily identify the following events happening to the ancilla-qutrit system: If the ancilla is in $\ket{0}_a$, the qutrit state is left unchanged with probability
\grayone{$1  -  {\alpha^2}/{4} -  {\beta^2}/{2} $} or it undergoes an $X_q$ bit-flip error with probability 
\graytwo{${\beta^2}/{4} $}. When the ancilla is instead in $\ket{1}_a$, the qutrit state is left unchanged in the loss state $\ket{2}\bra{2}_q$ with probability \graysix{$1 - {\beta^2}/{4}$}. 

We can also identify the origin of the false negative and false positive events: From $\Lambda_0$ we see that the qutrit will be projected on the loss state $\ket{2}\bra{2}_q$ with probability \graythree{${\beta^2}/{4} $} while the ancilla will be in the no-loss detected state $\ket{0}_a$. This corresponds to a false negative event whose origin can be traced back to the single qubit overrotation $R$ of Eq.~\eqref{SIEqn:CorrelatedSingleRotationChannel}.

From $\Lambda_1$ we see that when the qutrit is generated in the computational space by $\ket{0}_q$ and $\ket{1}_q$, the ancilla will be found in the loss detected state $\ket{1}_a$. In particular, the qutrit will be left unchanged with probability \grayfive{${\beta^2}/{4} $} and it will undergo an $X_q$ bit-flip error with probability \grayfour{${\alpha^2}/{4}$}. These events correspond to false positive events whose origin can be traced back to the single qubit overrotation $R$ and to the correlated overrotation $U_\text{corr}$ of Eq.~\eqref{SIEqn:CorrelatedSingleRotationChannel}. 

The previous considerations on the Choi operators $\Lambda_0$ and $\Lambda_1$ can be made more precise by computing explicitly the process in Eq.~\eqref{eqn_supp_coherent_channel}  with the help of Eqs.~\eqref{SIEq:CorrelatedNoiseModel}, \eqref{eqn_rotation_x_a} and \eqref{eqn_rotation_x_q} and by retaining only the terms that can be written in the Kraus form $P\rho P^\dag$ where $P$ is a Pauli operator. In this way, we can approximate the channel in Eq.~\eqref{eqn_supp_coherent_channel} as 
\begin{equation}\label{supp_eqn_inchoerent_channel}
\begin{split}\rho \mapsto &  p_a\ P_{01}\rho P_{01}^\dag + p_b\ X_q\rho X_q  +  p_c\ X_a X_q\rho X_q X_a + p_d\ X_a P_{01}\rho  P_{01}^\dag X_a \\ &+  q_a \  X_a \ket{2}\bra{2} \rho \ket{2}\bra{2} X_a + q_b \ \ket{2}\bra{2} \rho \ket{2}\bra{2} 
\end{split}
\end{equation}
where $\rho$ is the density matrix of the whole ancilla and qutrit system, $P_{01} = 1 - \ket{2}\bra{2}_q$ is the projector on the computational space $\{\ket{0}_q, \ket{1}_q\}$ of the qutrit and the probabilities take the form
\begin{gather}
p_a=\sin^2\alpha \sin^4\beta + \cos^2\alpha \cos^4\beta \sim 1 - {\alpha^2}/{4} - {\beta^2}/{2}   \\
p_b={\sin^2\beta}/{4} \sim {\beta^2}/{4} \\ 
p_c=\sin^2\alpha \cos^4\beta + \cos^2\alpha \sin^4\beta \sim {\alpha^2}/{4} \\
p_d = {\sin^2\beta}/{4} \sim {\beta^2}/{4} \\ 
q_a= \cos^2\left({\beta}/{2}\right) \sim 1 - {\beta^2}/{4} \\ 
q_b= \sin^2\left({\beta}/{2}\right)  \sim  {\beta^2}/{4}.
\end{gather}

The channel in Eq.~\eqref{supp_eqn_inchoerent_channel} can be then implemented in the following way:
\begin{enumerate}
\item If the ancilla is in $\ket{0}_a$ we
\begin{enumerate}
\item leave the qutrit state in the computational space with probability \grayone{$1  - {\beta^2}/{2}  - {\alpha^2}/{4} $};
\item apply an $X_q$ bit-flip error to the qutrit with probability \graytwo{${\beta^2}/{4} $};
\item apply an $X_q$ bit-flip error to the qutrit and an $X_a$ bit-flip error to the ancilla with probability \grayfour{${\alpha^2}/{4} $} (corresponding to a false positive event from the correlated overrotation);
\item leave the qutrit state as it is and flip the ancilla with probability \grayfive{${\beta^2}/{4} $} (corresponding to a false positive event from the single rotations).
\end{enumerate}

\item If the ancilla is in $\ket{1}_a$ we
\begin{enumerate}
\item leave the qutrit state in the loss state $\ket{2}_q$ with probability \graysix{$1 - {\beta^2}/{4}$};
\item flip the ancilla to the no-loss detection state  $\ket{0}_a$ with probability \graythree{${\beta^2}/{4} $} (corresponding to a false negative from the single rotations).
\end{enumerate}
\end{enumerate}
The comparison between the coherent channel in Eq.~\eqref{SIEqn:CorrelatedSingleRotationChannel} and the effective Clifford channel previously described is shown in Fig.~\ref{supp_fig_coherent_incoherent} and in Fig.~\ref{fig_coherent_incoherent} of the main text.

\begin{figure*}
    \centering
    \includegraphics[width=0.9\textwidth]{Figures/S12_zero_loss.pdf}
    \caption{\textbf{Comparison between the coherent and incoherent implementations of the faulty QND loss-detection unit in the case of no losses.} \textbf{(a)} Logical error rate as a function of the correlated overrotation rate $p_1$ for the parameter $p_2 = 0.045$ obtained from the experimental data. \textbf{(b)} Logical error rate as a function of the correlated overrotation rate $p_2$ for the parameter $p_1 =$ 2.47e-4 obtained from the experimental model.}
        \label{supp_fig_coherent_incoherent}
\end{figure*}  


\section{Losses in the 7-qubit code}
\label{SISec:ColorCode}
In this section, we discuss the correction from losses for the 7-qubit color code, in the ideal scenario of perfect QND loss detection and stabilizer measurements. We also assume that losses occur on each qubit independently with loss probability~$p$. 

A loss event is correctable if the density matrix of the losses is fully mixed or, more generally, it does not contain any information on the encoded logical state. With this criterion, we can then check the loss events that can be corrected. Obviously, the event (happening with probability $P_0 = (1-p)^7$) where no loss occurs is  correctable. The events where one loss occurs are also correctable. For showing this, let us consider for instance the encoded $\ket{0_L}$ state 
\begin{equation}\label{supp_eqn_logical_zero_loss}
\ket{0_L} \sim (\mathds{1} + S_{x}^{(1)})(\mathds{1} + S_{x}^{(2)})(\mathds{1} + S_{x}^{(3)})\ket{0}^{\otimes 7}
\end{equation}
where $S_{x}^{(j)}$ are the stabilizer generators and let us suppose that the loss affects the qubit $q_1$ (see Fig.~\ref{Fig:7QubitCode}a of the main text). By introducing the two orthogonal states $\ket{\chi_0} = P_{x}^{(2)} P_{x}^{(3)}\ket{0}^{\otimes 6}$ and  $\ket{\chi_1} = X_2 X_3 X_4 P_{x}^{(2)} P_{x}^{(3)}\ket{0}^{\otimes 6}$ (where $P_{x}^{(j)}  = \mathds{1} + S_{x}^{(j)}$ with $j=2,3$ are chosen because the loss does not belong to $S_{x}^{(j)}$), the state $\ket{0_L}$ can be written  explicitly as
\begin{equation} 
\ket{0_L} \sim \ket{0_1} \ket{\chi_0} + \ket{1_1} \ket{\chi_1}.
\end{equation}
As $\ket{\chi_0}$ and  $\ket{\chi_1}$ are orthogonal, the reduced density matrix of the loss $q_1$ obtained by tracing out the 6 other qubits will be $\rho_1 \sim \ket{0_1}\bra{0_1}+ \ket{1_1}\bra{1_1} $, i.e. it will be fully mixed. Therefore the events with one loss (happening with probability $P_1 = 7p(1-p)^6$) can be correctable. A similar reasoning applies to all the events where two losses happen  ($P_2 = 21 p^2(1-p)^5$) and to the events where three losses that do not form a logical operator happen as well.  The events with three losses that form a logical operator are instead not correctable. There are precisely 7 of such events (corresponding to the logical operators $\mathcal{L} = \{[1,2,5], [1,3,6], [1,4,7],[2,3,7],[4,3,5],[5,6,7], [2,4,6]\}$ in Fig.~\ref{Fig:7QubitCode}a of the main text). The last one ($ [2,4,6] $) is given by the product of the logical operator acting on all the 7 qubits multiplied by all the 3 stabilizer generators. This implies that the probability to successfully recover the logical state is $P_3 = [\binom{7}{3} - 7] p^3(1-p)^4 = 28 p^3(1-p)^4$. In the case of four losses, we have that in 7 cases out of $\binom{7}{4} = 35$ the reduced density matrix of the losses does not depend on the encoded logical state. These cases correspond to the losses happening on the qubits of the stabilizer generators and their products and are given by 
\begin{equation}
\mathcal{S} = \{[1, 2, 3, 4], [2, 3, 5, 6], [3, 4, 6, 7], [1, 4, 5, 6], \linebreak[0] [1, 2, 6, 7], [2, 4, 5, 7], [1, 3, 5, 7]\}.
\end{equation}

This can be shown by considering for instance four losses happening on the stabilizer $[1, 2, 3, 4]$. A bit of algebra shows that the logical states $\ket{0_L}$ and $\ket{1_L}$ can be written as
\begin{gather}
\ket{0_L} =  \ket{G}\ket{000} + X_2 X_3\ket{G}\ket{110} + X_3 X_4 \ket{G}\ket{011} + X_2 X_4\ket{G}\ket{101} \\
\ket{1_L} =  \ket{G}\ket{111} + X_2 X_3\ket{G}\ket{001} + X_3 X_4 \ket{G}\ket{100} + X_2 X_4\ket{G}\ket{010}.
\end{gather}
where $\ket{G} = \ket{0000} + \ket{1111}$ is a GHZ state of the qubits 1, 2, 3, 4 where the losses happen. Tracing on the qubits 5, 6, 7 transforms any logical state $\ket{\psi_L} = c_0 \ket{0_L} + c_1 \ket{1_L}$ into a mixture with equal probabilities of the four states $\{\ket{G}, X_2 X_3\ket{G},  X_3 X_4 \ket{G}, X_2 X_4\ket{G}\}$ that is independent on the coefficients $c_0$ and $c_1$. Finally, no event with five, six or seven losses can be corrected. The total probability of a successful correction is given by the sum of all the probabilities $P_j$ and reads
\begin{equation}\label{prob_success}
\begin{split}
p_\text{success} & = (1-p)^7 + 7p(1-p)^6 + 21 p^2(1-p)^5 + 28 p^3(1-p)^4 + 7p^4(1-p)^3 \\
& = 1 -7 p^3+21 p^5 -21 p^6 + 6 p^7.
\end{split}
\end{equation}
